RECALL: REpresentation-aligned Catastrophic-forgetting ALLeviation via Hierarchical Model Merging

We unveil that internal representations in large language models (LLMs) serve as reliable proxies of learned knowledge, and propose RECALL, a novel representation-aware model merging framework for continual learning without access to historical data. RECALL computes inter-model similarity from layer-wise hidden representations over clustered typical samples, and performs adaptive, hierarchical parameter fusion to align knowledge across models. This design enables the preservation of domain-general features in shallow layers while allowing task-specific adaptation in deeper layers. Unlike prior methods that require task labels or incur performance trade-offs, RECALL achieves seamless multi-domain integration and strong resistance to catastrophic forgetting. Extensive experiments across five NLP tasks and multiple continual learning scenarios show that RECALL outperforms baselines in both knowledge retention and generalization, providing a scalable and data-free solution for evolving LLMs.

==> sections/Experiments_setup.tex <==


\begin{comment} 
    实验环境（使用了什么GPU），数据集（split和评估指标）、模型、pipeline(训练用llama-factory,评测试用opencompass)、baseline，
    ---
在我们的实验中，我们使用llama2-7B-chat模型作为后续微调和权重融合的基础模型，并通过在8张NVIDIA V100 GPUs上进行Lora微调以获得专家模型。我们考虑了在知识融合和持续学习中一种具有挑战的设置，使用了包括文本分类，阅读理解以及文本生成等涵盖了多个领域和任务的数据集，并在这些数据集上对不同的baseline以及xxx算法进行了评测。
    ---
\end{comment}
In our experiment, we selected the Llama-2-chat-7B model (\citealp{touvron2023llama}) as the source model for fine-tuning and weight merging. Expert models were fine-tuned with LoRA (\citealp{hu2022lora}) on 8 NVIDIA V100 GPUs. Considering a challenging experimental setup in knowledge fusion and continual learning, we selected datasets from multiple domains and tasks to verify the universality of the method we proposed, including text classification, single-choice, and text generation. To evaluate the performance of XXX, we conducted experiments on these datasets and compared the results with multiple baselines. The experimental setup is detailed below.
\subsection{Datasets}
\begin{itemize}
\item[$\bullet$] \textbf{SST-2} (\citealp{socher-etal-2013-recursive})\textbf{:}A binary sentiment classification dataset consisting of movie reviews labeled as either positive or negative.
\item[$\bullet$] \textbf{SQuAD2.0} (\citealp{rajpurkar-etal-2016-squad}; \citealp{rajpurkar-etal-2018-know})\textbf{:}A reading comprehension dataset that combines questions with and without answerable contexts to evaluate model robustness in question answering.
\item[$\bullet$] \textbf{MedMCQA} (\citealp{pmlr-v174-pal22a})\textbf{:}A large-scale, multiple-choice question answering dataset derived from Indian medical entrance exam questions, designed to assess domain-specific reasoning capabilities.
\item[$\bullet$] \textbf{RACE} (\citealp{lai-etal-2017-race})\textbf{:}A reading comprehension dataset collected from English exams for middle and high school students in China, requiring reasoning and inference over long passages.
\item[$\bullet$] \textbf{IWSLT2017-en-fr} (\citealp{cettolo-etal-2017-overview})\textbf{:}A machine translation benchmark consisting of English-to-French sentence pairs from TED talks, commonly used for evaluating translation models.
\end{itemize}

\begin{comment}
    sst2
    squad20
    medmcqa
    race
    iwslt2017-en-fr
    这部分介绍一下使用的数据集，附录里面要给example表明每个数据集的prompt是怎么样的，以及split的划分,以及评估指标，是acc还是rougeL。
\end{comment}
\subsection{Pipeline}  

\begin{comment}
    这部分介绍微调和评测时使用的框架，就是llama-factory和opencompass。附录中需要包含微调时使用的参数,Opencompass使用vllm加速都要提一下。
\end{comment}
\begin{itemize}
\item[$\bullet$] \textbf{Fine-tuning:} We utilize llama-factory(\citealp{zheng2024llamafactory}) for instruction tuning. This framework supports various parameter-efficient fine-tuning methods such as LoRA(\citealp{hu2022lora}) and QLoRA(\citealp{dettmers2023qlora}), and provides flexibility in handling different dataset formats, making it easy to customize training pipelines.
\item[$\bullet$] \textbf{Evaluation:} Model evaluation is performed using OpenCompass(\citealp{2023opencompass}), which integrates a wide range of standardized benchmarks and provides a unified evaluation interface to ensure the reliability and reproducibility of results. In addition, vLLM(\citealp{kwon2023efficient}) is employed to serve models during inference, offering high throughput and low latency for efficient evaluation.
\end{itemize}
\subsection{Baseline}



==> sections/Introduction.tex <==
\begin{comment} 
Bibi, Microwave TEST!!
大语言模型（LLM）[1,2,3,4,5,6,7]在近几年取得了令人印象深刻的成果，已经在各种下游任务上取得了显著的突破，包括问答，生成，数学推理等，并被应用到诸如对话机器人、AI业务代理、推荐系统等实际场景中。通常情况下，一个具有专业能力的LLM需要经过预训练（PT）、SFT有监督微调等阶段（SFT）。在预训练阶段，LLM在大量通用数据上进行无监督训练[2,5]。在有监督微调阶段，模型在某些特定领域的有标签数据上进行有监督学习，使其适应特定的下游任务[8,9]。
虽然SFT可以使得LLM在特定任务上的性能得到提高，在某些任务上甚至可以达到人类的水平，但LLM与人类智能最大的不同在于，人类可以在学习新知识的同时极大地保留先前学习到的知识，而LLM在SFT后却会表现出在其他任务性能上的严重退化。这种现象被称作神经网络的灾难性遗忘（Catastrophic Forgetting），指由训练中数据分布变化导致的神经网络参数变化，使得神经网络在其他任务上的性能显著下降[10, 11,12,13,14]。）

灾难性遗忘对于需要多任务学习或多领域应用的模型来说是一个重大挑战，因为理想的模型应该能够在学习新任务的同时保持对旧任务的良好性能，从而同时具有专家和全才的能力(brown2020language, wei2021finetuned)。


\end{comment}
Large language models (LLM) have achieved impressive progress in recent years and have made significant breakthroughs in various downstream tasks, including question answering, text generation, mathematical reasoning, and have become the key technology for implementing some of the most advanced AI applications (\citealp{devlin2018bert}; \citealp{touvron2023llama}; \citealp{achiam2023gpt}; \citealp{raffel2020exploring}). Typically, multiple training stages, including pre-training (PT), supervised fine-tuning (SFT), and other stages, are required for an LLM to acquire world knowledge and improve specific abilities. At first stage, an LLM is pre-trained on a large mount of general-purpose data through an unsupervised process (\citealp{brown2020language}; \citealp{touvron2023llama}). Then at the SFT stage, the pre-trained model does supervised learning on labeled data of certain specific fields to adapt to corresponding downstream tasks (\citealp{wei2021finetuned}; \citealp{ouyang2022training}).

Although through supervised fine-tuning a language model can improve the performance on specific tasks and even reach the level of human beings, the biggest difference between LLM and human-level intelligence is that human beings can greatly retain the previously learned knowledge while learning new knowledge, while LLM will show serious performance degradations on other tasks after fine-tuning. This phenomenon is called catastrophic forgetting (CF) of neural networks, which refers to the change in model parameters caused by the drift in data distribution in training, and results in losing previous capabilities (\citealp{1989Catastrophic}; \citealp{2016Overcoming}; \citealp{8107520}).
As an ideal model should be able to adjust to new tasks while maintaining good performance on previous tasks, catastrophic forgetting has become a significant challenge for machine learning communities. (\citealp{brown2020language}, \citealp{wei2021finetuned}).
\begin{comment}
    <CHECK>

为了解决这一挑战，近年来有许多方法被提出，如图1(Fig 1)所示。这些方法可以分为三类，但在大语言模型微调的背景下，这些方法仍存在很多缺陷。(a) 基于正则化的方法通过在损失函数中增加正则项来惩罚在持续学习中产生的知识变化。面对复杂的NLP任务场景和长序列任务时，这种方法往往难以满足需求（2021Continual；2016Overcoming；8107520；wang-etal-2023-orthogonal） (b) 基于数据replay的方法通过在缓冲区中保存过往任务的samples并在新一轮训练中访问这些samples来维持模型的能力。但实际情况中过往数据并不总是可以获取，而且这种方法也会存在潜在的隐私问题(NIPS2017_f8752278;2016iCaRL;2019Adversarial;isele2018selective);(3) 模型动态扩展方法训练多个不同的模块来帮助模型抵抗灾难性遗忘，在推理时依据明确的任务id或者路由模块来决定使用其中的一个或多个模块隔离任务间的知识干扰。但这会使模型在不断的训练中规模变大，而且在实际场景中往往缺乏可靠的任务id或者边界。（rusu2016progressive；fernando2017pathnet；tian2024hydralora；zhu2024llama）

<CHECK>
\end{comment}

\textbf{<TOCHECK>}

To mitigate catastrophic forgetting, numerous approaches have been proposed in recent years. As shown in Fig. 1, these approaches can be classified into three categories. However, in the context of large language model fine-tuning, these methods still encounter significant limitations. (a) Regularization-based methods penalize knowledge changes generated during continual learning by introducing regularization terms to the loss function (\citealp{2021Continual}; \citealp{2016Overcoming}; \citealp{8107520}; \citealp{wang-etal-2023-orthogonal}), which are often difficult to meet the requirements of complex tasks and scenarios of long task sequences. (b) Replay-based methods maintain the model's capabilities by saving samples of previous tasks in a buffer and accessing these samples in a new round of fine-tuning (\citealp{NIPS2017_f8752278}; \citealp{2016iCaRL}; \citealp{2019Adversarial}; \citealp{Isele_Cosgun_2018}). But in practice, it is not always able to save or access previous samples, while these approaches also raise potential privacy issues. (c) Architecture-based methods train multiple different modules to help the model resist catastrophic forgetting, and use one or more of them to isolate the knowledge interference between tasks according to the explicit task ID or routing module during inference (\citealp{rusu2016progressive}; \citealp{fernando2017pathnet}; \citealp{tian2024hydralora}). However, such methods essentially lead to continual growth of model scale during continual training. Besides, in practical applications reliable task ID or unambiguous may not be feasible.

\textbf{<TOCHECK>}


\begin{comment}
    （4） 模型融合/参数融合(model fusion/parameter merging)通过将具有不同能力的模型的参数加权平均来获得具有多种才能的模型，相比于其他方法，模型融合不依赖于序列学习的模式，也不依赖于模型本身的训练方式，是一种更通用的抗遗忘范式。但不幸的是，现有方法对模型融合的设计比较简单，缺少对不同模型参数更细致的分析。(LM-Cocktail,model soup, LLLM-Blender, ...还有挺多的)(xiao2023lm; wortsman2022model; jiang2023llm; Wortsman_2022_CVPR)
\end{comment}


\textbf{<EMBEDDING>}
\begin{comment}
ref:
[1]Investigating Forgetting in Pre-Trained Representations Through Continual Learning (2023Investigating)
[2]Embedding Trajectory for Out-of-Distribution Detection in Mathematical Reasoning (wang2024embedding)
[3]Semantic Drift Compensation for Class-Incremental Learning (9156964)
[4]Alleviating representational shift for continual finetuning (9857197)
[5]learning without forgetting ??(8107520)
[6]Overcoming catastrophic forgetting in neural networks ??(2016Overcoming)
[7]Representation Alignment for Generation: Training Diffusion Transformers Is Easier Than You Think (yu2025representation)
[8]The Geometry of Concepts: Sparse Autoencoder Feature Structure (li2024the)
[9]Understanding LLM Embeddings for Regression (Tang2024UnderstandingLE)
[9]The Representation Landscape of Few-Shot Learning and Fine-Tuning in Large Language Models (Doimo2024TheRL)

除了经典的序列式的持续学习外，我们还考虑了另一种持续学习的场景，即如何整合多个专家模型的能力以获得更强大的通用模型。In this work, 我们希望能结合大语言模型的可解释性，提供一种更加全面且直观的方法。先前的工作表明，神经网络的灾难性遗忘与数据表征的变化密不可分(9156964; 9857197; 2023Investigating)，如Fig 2所示，在训练前后同一批数据的表征会改变，我们进一步分析了transformer模型的层间的表征漂移(representation drift)，并利用多个特定层表征的区别构建了一种对不同专家模型能力的表示方法，拥有相似能力的模型的能力表示向量将会更相近。最后，我们计算模型间能力的相似度以获取参数融合时的权重。

为了验证\textbf{<FILL>}的有效性，我们在多种混合任务的数据集上进行了训练，....数据集上进行了实验。\textbf{<FILL>}在大量且广泛的数据集上展现出了卓越的性能，这也证明了...的普适性，尤其是在LLM的SFT任务上，可以有效的缓解灾难性遗忘现象。这说明...可以被应用到更广泛的抗遗忘任务上。


我们的方法提供了3个优点：<TOFILL>
该研究不仅为LLM的持续学习研究做出巨大贡献，也在一定程度上揭示了模型表征与模型可解释性之间的关系。
(In summary, the primary contributions of this paper can be summarized as follows：
（1）我们提出了一个新颖？的....框架，可以广泛且有效地缓解LLM微调产生的灾难性遗忘问题，并且不需要...(比如数据重放)
（2）？？？我们从多元数据表征分布的角度探讨了不同微调数据对模型遗忘的影响，为模型可解释性提供了新的视角。
（3）我们在大量基准实验中证明了该方法在泛化与抗遗忘任务上的有效性和优越性。
\end{comment}

In addition to the classical scenario of sequential continual learning, we also consider another scenario: how to integrate the capabilities of multiple models to obtain a powerful and general model. In this work, we hope to provide a more comprehensive and intuitive approach by incorporating the interpretability of large language models. Previous work has shown that catastrophic forgetting in neural networks is inseparable from changes in data representation (\citealp{9156964}; \citealp{9857197}; \citealp{2023Investigating}). As shown in Fig. 2, the representation of the same batch of data will change before and after training. We further analyze the representation drift between layers of transformer models. And a method for representing the capabilities of different models is constructed by using the differences between the representations of multiple specific layers. Under our distance metric, the representation vectors of models with similar capabilities will be closer together. Finally, we calculate the weights for parameter merging by comparing the similarities between models.


\begin{comment}
语义 or 任务
[1]What does BERT learn about the structure of language? (jawahar:hal-02131630)
[2]BERT rediscovers the classical NLP pipeline (Tenney2019BERTRT )      
[3]The Representation Landscape of Few-Shot Learning and Fine-Tuning in Large Language Models (Doimo2024TheRL)
[4]Investigating Forgetting in Pre-Trained Representations Through Continual Learning (2023Investigating)
\end{comment}


==> sections/Preliminaries.tex <==
\begin{comment} 
Supervise Fine-tuning:有监督微调的输入由一组带标签的数据组成$D={(x_i,y_i)}_{i=1}^{N}$，旨在通过调整模型参数来增强模型有效响应指令的能力。在形式上，可以将SFT过程表示为：
$\theta^*=\arg\min_{\theta}E_{(x,y)~D}[-L(f_{\theata}(x),y]\approx\arg\min_{\theta}\sum_{i=1}^N-logP(y_i|)$
其中，...
Continual Learning：持续学习的目标是为了提高模型在连续学习中获取知识的能力并缓解由数据分布变化导致的灾难性遗忘问题。通常，这意味着模型要顺序地在一系列任务上进行训练$D={D_1,D_2,...}$，其中...。在每个阶段t，模型不仅要保证在$D_t$上有足够的性能，还要尽可能保持在之前任务上$D_{<t}$上性能不下降。因此，我们可以形式化地写出持续学习的目标：

其中...
然而，由于在LLM微调中，过往数据往往由于隐私问题或是缺少来源而不可知，并且每个$D_i$间不存在类变化（除非涉及到词表扩展）、缺少明显的领域或者任务界限，多数传统的持续学习方法并不能很好的应用到LLM的持续微调中。（这里应该说的更简洁点吗？比如然而，当前的持续学习方法由于其严格的约束，总是遇到实际的限制和挑战，这在现实生活场景中很难实现）。
因此，我们考虑一种泛用性更强，且更实际的场景：（讲述多模型聚合场景）
\end{comment}
\textbf{Supervised fine-tuning (SFT)} aims to enhance the model's ability to respond effectively to specific instructions by adjusting its parameters. The model is to be fine-tuned by a dataset of labeled samples $\mathcal D=\{(\boldsymbol{x}_i,\boldsymbol{y}_i)\}_{i=1}^{N}$, in which
$\boldsymbol{x}_i$ represents the input and $\boldsymbol{y}_i$ represents the corresponding expected output. Formally, SFT can be formulated as the process of optimizing the model parameters $\boldsymbol{\theta}$ with the minimum log-likelihood loss as follows:\\
\begin{equation}
\label{SFT Process}
\begin{aligned} \boldsymbol{\theta}^*&=\arg\min_{\boldsymbol{\theta}}\mathbb{E}_{(\boldsymbol{x},\boldsymbol{y})\sim\mathcal D}[\mathcal L(\mathcal M_{\boldsymbol{\theta}}(\boldsymbol{x}),\boldsymbol{y})] \\
&\approx\arg\min_{\boldsymbol{\theta}}\sum_{i=1}^N\mathcal L(\mathcal M_{\boldsymbol{\theta}}(\boldsymbol{x}_i),\boldsymbol{y}_i)\\
&=\arg\min_{\boldsymbol{\theta}}\sum_{i=1}^N-\log \mathbf{P}_{\boldsymbol{\theta}}(\boldsymbol{y}_i|\boldsymbol{x}_i)
\end{aligned}
\end{equation}
where $\mathcal M_{\boldsymbol{\theta}}(\bullet)$ denotes the model's output under parameter $\boldsymbol{\theta}$, and $\mathcal L(\bullet,\bullet)$ denotes the loss function, which is equivalent to the log-likelihood probability in our description.
\\\textbf{Continual learning(CL)} aims to improve the model's ability to acquire knowledge in continuous learning and alleviate catastrophic forgetting (CF) caused by drifts of data distribution. Generally, this means that the model is trained sequentially on a series of $K$ datasets $\boldsymbol{\mathcal D}=\{\mathcal D_t\}_{t=1}^{K}$, each subset $\mathcal D_t$ contains $N_t$ samples $\{(\boldsymbol{x}_i^t,\boldsymbol{y}_i^t)\}_{i=1}^{N_t}$. At each stage $t$, the model is expected not only to improve its performance on task $\mathcal D_t$, but also to maintain the performances on the previous datasets $\boldsymbol{\mathcal D}_{<t}=\{\mathcal D_i\}_{i<t}$ without degradation. Therefore, the optimization objective of continual learning can be formulated as follows:\\
\begin{equation}
\label{CL Process}
\begin{aligned} \boldsymbol{\theta}^*&=\arg\min_{\boldsymbol{\theta}}\mathbb{E}_{(\boldsymbol{x},\boldsymbol{y})\sim\boldsymbol{\mathcal D}}[\mathcal L(\mathcal M_{\boldsymbol{\theta}}(\boldsymbol{x}),\boldsymbol{y})] \\
&\approx\arg\min_{\boldsymbol{\theta}}\sum_{t=1}^{K}\sum_{i=1}^{N_t}\mathcal L(\mathcal M_{\boldsymbol{\theta}}(\boldsymbol{x}^t_i),\boldsymbol{y}^t_i)\\
&=\arg\min_{\boldsymbol{\theta}}\sum_{t=1}^{K}\sum_{i=1}^{N_t}-\log \mathbf{P}_{\boldsymbol{\theta}}(\boldsymbol{y}^t_i|\boldsymbol{x}^t_i)
\end{aligned}
\end{equation}





\textbf{Model Merging} \\
\textbf{TODO} \\
\textbf{TODO} \\
\textbf{TODO} \\
